Measurement of the Double Beta Decay Half-life of 130Te with the NEMO-3 Detector

This Letter reports results from the NEMO-3 experiment based on an exposure of 1275 days with 661g of 130Te in the form of enriched and natural tellurium foils. The double beta decay rate of 130Te is found to be greater than zero with a significance of 7.7 standard deviations and the half-life is measured to be T1/2 = (7.0 +/- 0.9(stat) +/- 1.1(syst)) x 10^{20} yr. This represents the most precise measurement of this half-life yet published and the first real-time observation of this decay.

==> prl-CCauth.tex <==
\title{Measurement of the Double Beta Decay Half-life of \boldsymbol{$^{130}$}Te~with the NEMO-3 Detector}


\newcommand{\Lebedev}{Nuclear Physics Dept., Lebedev Physical Inst., Leninsky Prospect 53, 117924 Moscow, Russia}
\newcommand{\IHEP}{Inst. for High Energy Physics, Protvino, Moscow Region RU-140284, Russia}
\newcommand{\Texas}{Dept. of Physics, Univ. of Texas, 1 University Station, Austin, TX 78712}
\newcommand{\Wisconsin}{Physics Dept., Univ. of Wisconsin, Madison, WI 53706}
%\newcommand{\deceased}{Deceased.}
\newcommand{\LAL}{LAL, Universit\'e Paris-Sud 11,  CNRS/IN2P3, Orsay, France}
\newcommand{\IPHC}{IPHC-DRS, Universit\'e Louis Pasteur, CNRS, F-67037 Strasbourg, France}
%\newcommand{\INL}{INL, Idaho Falls, Idaho 83415, USA}
\newcommand{\INL}{INL, Idaho National Laboratory, Idaho Falls, Idaho 83415, USA}
\newcommand{\ITEP}{ITEP, Institute of Theoretical and Experimental Physics, 117259 Moscow, Russia}
%\newcommand{\ITEP}{ITEP, 117218 Moscow, Russia}
%  B. Cheremushkinskaya, 25, 117218 Moscow, Russia}
\newcommand{\UdB}{Universit\'e de Bordeaux, 
CENBG, UMR 5797, 
 F-33175 Gradignan, France}
%Centre d'Etudes Nucl\'eaires de Bordeaux Gradignan, UMR 5797, 
% F-33175 Gradignan, France}
\newcommand{\CNRS}{CNRS/IN2P3,  
CENBG, UMR 5797, 
 F-33175 Gradignan, France}
%Centre d'Etudes Nucl\'eaires de Bordeaux Gradignan, UMR 5797, 
% F-33175 Gradignan, France}
%\newcommand{\JINR}{JINR, 141980 Dubna, Russia}   
\newcommand{\JINR}{JINR, Joint Institute for Nuclear Research, 141980 Dubna, Russia}   
%\newcommand{\JINR}{Joint Institute for Nuclear Research, 141980 Dubna, Russia}
%\newcommand{\UCL}{Dept. of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT, UK}
%\newcommand{\UCL}{UCL, WC1E 6BT  London, UK}
\newcommand{\UCL}{University College London, London WC1E 6BT, United Kingdom}
\newcommand{\UMAN}{University of Manchester, Manchester M13 9PL, UK}
%\newcommand{\USMBA}{USMBA, Fes, Morocco}
\newcommand{\USMBA}{USMBA, Universit\'e Sidi Mohamed Ben Abdellah, 30000 Fes, Morocco}
\newcommand{\UTA}{University of Texas at Austin, Austin, Texas 78712-0264, USA}
\newcommand{\IEAP}{IEAP, Czech Technical University in Prague,  CZ-12800 Prague, Czech Republic}
\newcommand{\LPC}{LPC, ENSICAEN, Universit\'e de Caen, Caen, France}
\newcommand{\IFIC}{IFIC, CSIC - Universidad de Valencia, Valencia, Spain}
\newcommand{\UB}{Universitat Aut\`onoma de Barcelona, Spain}
\newcommand{\Saga}{Saga University, Saga 840-8502, Japan}
\newcommand{\LSCE}{LSCE, CNRS, F-91190 Gif-sur-Yvette, France}
\newcommand{\FMFI}{FMFI, Comenius University, SK-842 48 Bratislava, Slovakia}
\newcommand{\JU}{Jyv\"{a}skyl\"{a} University,  40351 Jyv\"{a}skyl\"{a}, Finland}
%\newcommand{\MHC}{MHC, South Hadley, Massachusetts 01075, USA}
\newcommand{\MHC}{MHC, Mount Holyoke College, South Hadley, Massachusetts 01075, USA}
%\newcommand{\CU}{FMP, Charles University in Prague, Prague, Czech Republic}
\newcommand{\CU}{Charles University in Prague, Faculty of Mathematics and Physics, CZ-12116 Prague, Czech Republic}
%\newcommand{\IC}{Imperial College of Science, Technology and Medicine, Prince Consort Road, London}
\newcommand{\IC}{Imperial College London, London SW7 2AZ, UK}
\newcommand{\HU}{Hanoi University of Science, Hanoi, Vietnam}
%\newcommand{\FNAL}{FNAL, Batavia, IL 60510 USA} 
%\newcommand{\dec}{Deceased}


\affiliation{\IPHC}
\affiliation{\LAL}
\affiliation{\INL}
\affiliation{\ITEP}
\affiliation{\UCL}
\affiliation{\UdB}
\affiliation{\CNRS}
\affiliation{\JINR}
\affiliation{\LPC}
\affiliation{\UMAN}
\affiliation{\USMBA}
\affiliation{\UTA}
\affiliation{\IEAP}
\affiliation{\IFIC}
\affiliation{\HU}
\affiliation{\Saga}
\affiliation{\LSCE}
\affiliation{\IC}
\affiliation{\FMFI}
\affiliation{\JU}
\affiliation{\MHC}
\affiliation{\CU}


%\author{J.~Argyriades}
%\affiliation{\LAL}
\author{R.~Arnold}
\affiliation{\IPHC}
\author{C.~Augier}
\affiliation{\LAL}
\author{\fbox{J.~Baker}}
\affiliation{\INL}
%\affiliation{\dec}
\author{A.S.~Barabash}
\affiliation{\ITEP}
\author{A.~Basharina-Freshville}\affiliation{\UCL}
\author{S.Blondel}\affiliation{\LAL}
\author{M.~Bongrand}
\affiliation{\LAL}
\author{G.~Broudin-Bay}
\affiliation{\UdB}\affiliation{\CNRS}
\author{V.~Brudanin}
\affiliation{\JINR}
\author{A.J.~Caffrey}
\affiliation{\INL}
\author{A.~Chapon}  
\affiliation{\LPC}
\author{E.~Chauveau}
\affiliation{\UdB}\affiliation{\CNRS}
\author{D.~Durand}  
\affiliation{\LPC}
\author{V.~Egorov}
\affiliation{\JINR}
%\author{N.~Fatemi-Ghomi}
%\affiliation{\UMAN}
\author{R.~Flack}
\affiliation{\UCL}
\author{X.~Garrido}
\affiliation{\LAL}
\author{J.~Grozier}\affiliation{\UCL}
\author{B.~Guillon}  
\affiliation{\LPC}
\author{Ph.~Hubert}
\affiliation{\UdB}\affiliation{\CNRS}
\author{C.M.~Jackson}  
\affiliation{\UMAN}
\author{S.~Jullian}
\affiliation{\LAL}
\author{M.~Kauer}
\affiliation{\UCL}
%\author{S.~King}
%\affiliation{\UCL}
\author{A.~Klimenko}
\affiliation{\JINR}
\author{O.~Kochetov}
\affiliation{\JINR}
\author{S.I.~Konovalov}
\affiliation{\ITEP}
\author{V.~Kovalenko}
\affiliation{\JINR}\affiliation{\UdB}
\author{D.~Lalanne}
\affiliation{\LAL}
\author{T.~Lamhamdi}
\affiliation{\USMBA}
\author{K.~Lang}
\affiliation{\UTA}
%\author{Y.~Lemi\`ere}
%\affiliation{\LPC}
\author{Z.~Liptak}
\affiliation{\UTA}
%\author{C.~Longuemare}
%\affiliation{\LPC}
\author{G.~Lutter}
\affiliation{\UdB}\affiliation{\CNRS}
\author{F.~Mamedov}
\affiliation{\IEAP}
\author{Ch.~Marquet}
\affiliation{\UdB}\affiliation{\CNRS}
\author{J.~Martin-Albo}
\affiliation{\IFIC}
\author{F.~Mauger}
\affiliation{\LPC}
\author{J.~Mott}\affiliation{\UCL}
\author{A.~Nachab}
\affiliation{\UdB}\affiliation{\CNRS}
%\author{I.~Nasteva}
%\affiliation{\UMAN}
\author{I.~Nemchenok}
\affiliation{\JINR}
\author{C.H.~Nguyen}  
\affiliation{\UdB}\affiliation{\CNRS}\affiliation{\HU}
\author{F.~Nova}
\affiliation{\UTA}
\author{P.~Novella}
\affiliation{\IFIC}
\author{H.~Ohsumi}
\affiliation{\Saga}
\author{R.B.~Pahlka}
\affiliation{\UTA}%\footnote{Current address FNAL, Batavia, IL 60510 USA}
\author{F.~Perrot}
\affiliation{\UdB}\affiliation{\CNRS}
\author{F.~Piquemal}
\affiliation{\UdB}\affiliation{\CNRS}
\author{J.L.~Reyss}
\affiliation{\LSCE}
\author{B.~Richards}\affiliation{\UCL}
\author{J.S.~Ricol}
\affiliation{\UdB}\affiliation{\CNRS}
\author{R.~Saakyan}
\affiliation{\UCL}
\author{X.~Sarazin}
\affiliation{\LAL}
\author{L.~Simard}
\affiliation{\LAL}
\author{F.~\v{S}imkovic}
\affiliation{\FMFI}
\author{Yu.~Shitov}
\affiliation{\IC}
\author{A.~Smolnikov}
\affiliation{\JINR}
\author{S.~S\"{o}ldner-Rembold}
\affiliation{\UMAN}
\author{I.~\v{S}tekl}
\affiliation{\IEAP}
\author{J.~Suhonen}
\affiliation{\JU}
\author{C.S.~Sutton}
\affiliation{\MHC}
\author{G.~Szklarz}
\affiliation{\LAL}
\author{J.~Thomas}
\affiliation{\UCL}
\author{V.~Timkin}
\affiliation{\JINR}
\author{S.~Torre}\affiliation{\UCL}
\author{V.I.~Tretyak}
\affiliation{\JINR}
%\footnote{To whom all correspondence should be addressed.}
\author{V.~Umatov}
\affiliation{\ITEP}
\author{L.~V\'{a}la}
\affiliation{\IEAP}
\author{I.~Vanyushin}
\affiliation{\ITEP}
\author{V.~Vasiliev}
\affiliation{\UCL}
\author{V.~Vorobel}
\affiliation{\CU}
\author{\fbox{Ts.~Vylov}}
\affiliation{\JINR}
%\affiliation{\dec}
\author{A.~Zukauskas}
\affiliation{\CU}


\collaboration{The NEMO-3 Collaboration}
\noaffiliation

\date{\today}

